Allocate Marginal Reviews to Borderline Papers Using LLM Comparative Ranking

This paper argues that large ML conferences should allocate marginal review capacity primarily to papers near the acceptance boundary, rather than spreading extra reviews via random or affinity-driven heuristics. We propose using LLM-based comparative ranking (via pairwise comparisons and a Bradley--Terry model) to identify a borderline band \emph{before} human reviewing and to allocate \emph{marginal} reviewer capacity at assignment time. Concretely, given a venue-specific minimum review target (e.g., 3 or 4), we use this signal to decide which papers receive one additional review (e.g., a 4th or 5th), without conditioning on any human reviews and without using LLM outputs for accept/reject. We provide a simple expected-impact calculation in terms of (i) the overlap between the predicted and true borderline sets ($\rho$) and (ii) the incremental value of an extra review near the boundary ($\Delta$), and we provide retrospective proxies to estimate these quantities.

==> sections/07_call_to_action.tex <==
\section{Call to Action}
\label{sec:call-to-action}
We propose a two-step rollout that avoids affecting assignments until the signal is validated.
This requires reallocating existing marginal review capacity, not creating new reviews.

\textbf{Step 1 (NeurIPS 2026 pilot, shadow mode).}
Run the LLM pairwise-comparison pipeline over all submitted papers to estimate $\rho$ and $\Delta$, but do \emph{not} use it to assign extra reviews.
After decisions are finalized, evaluate the predicted borderline band against outcomes and report the achieved $\rho$, runtime, and sensitivity to the band fraction.
Define explicit success criteria (e.g., $\rho$ above a random baseline by a fixed margin, positive $\Delta$ with a non-overlapping confidence interval, and acceptable runtime/cost) before proceeding beyond shadow mode.
Report distributional audits before any live use: because LLM reliability can vary by subfield, writing style, and language proficiency, the shadow-mode pilot should report overlap $\rho$ stratified by area (subject category) and it should report the rate at which different strata would receive $+1$ reviews under the policy relative to a random baseline.
These stratified audits are most informative at large scale (e.g., $N\approx 30{,}000$ submissions), where statistical power remains adequate even after partitioning into multiple fields and subfields.
For a NeurIPS-scale pilot, the NeurIPS Board should allocate a small operational budget (on the order of \$\NeuripsPilotBudgetDollars{}) to cover LLM usage and engineering time to integrate with OpenReview.
Organizers should use an enterprise deployment that does not retain submitted data or use it for model training.

\textbf{Step 2 (ICLR 2027 deployment).}
Implement the full system using the following steps:
\begin{enumerate}
\item Specify the borderline center (acceptance percentile) based on the expected acceptance rate, e.g., center at the $c=1-\TargetAcceptanceRate{}$ percentile of the comparative ranking.
\item Run the LLM pairwise-comparison pipeline over all papers, fit the Bradley--Terry model, and compute a total ordering.
We will open source the code to run the LLM-based paper ranking.
\item Define the borderline band as a two-sided interval centered at the estimated boundary, with width equal to the number of papers that can receive one additional review under the fixed extra-review capacity (i.e., the number of ``extra'' review slots above the stated minimum).
\item Integrate with OpenReview by assigning each paper a required minimum $r_{\min}$ reviews (typically $r_{\min}=3$ for most papers) and $r_{\min}+1$ for papers in the borderline set, while preserving conflicts, affinity constraints, and reviewer load balancing.
This uses the existing AC adjustment window for any manual swaps or exceptions.
\end{enumerate}

For an ICLR 2027 deployment, the ICLR Board should allocate a small operational budget (on the order of \$\NeuripsPilotBudgetDollars{}) to cover LLM usage and engineering time to integrate with OpenReview.

